The State of Pilot Study Reporting in Crowdsourcing: A Reflection on Best Practices and Guidelines

Pilot studies are an essential cornerstone of the design of crowdsourcing campaigns, yet they are often only mentioned in passing in the scholarly literature. A lack of details surrounding pilot studies in crowdsourcing research hinders the replication of studies and the reproduction of findings, stalling potential scientific advances. We conducted a systematic literature review on the current state of pilot study reporting at the intersection of crowdsourcing and HCI research. Our review of ten years of literature included 171 articles published in the proceedings of the Conference on Human Computation and Crowdsourcing (AAAI HCOMP) and the ACM Digital Library. We found that pilot studies in crowdsourcing research (i.e., crowd pilot studies) are often under-reported in the literature. Important details, such as the number of workers and rewards to workers, are often not reported. On the basis of our findings, we reflect on the current state of practice and formulate a set of best practice guidelines for reporting crowd pilot studies in crowdsourcing research. We also provide implications for the design of crowdsourcing platforms and make practical suggestions for supporting crowd pilot study reporting.

==> figures/FIG-CORPUS.tex <==

\begin{figure*}[t]
\begin{minipage}[b]{0.5\textwidth}
\small
\begin{tabularx}{\textwidth}{lX}%
\toprule%
    Year & Publications \\
\midrule%
    2012 & \input{years/2012} \\
    2013 & \input{years/2013} \\
    2014 & \input{years/2014} \\
    2015 & \input{years/2015} \\
    2016 & \input{years/2016} \\
    2017 & \input{years/2017} \\
    2018 & \input{years/2018} \\
    2019 & \input{years/2019} \\
    2020 & \input{years/2020} \\
    2021 & \input{years/2021} \\
\bottomrule%
\end{tabularx}%
\caption{Research articles reporting crowd pilot studies in the ACM Digital Library and HCOMP proceedings (2012 -- 2021).}
\label{tab:publications}%
\end{minipage}%
\begin{minipage}[b]{0.5\textwidth}
\begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{figures/images/pYearPilotStudies.png}
    \subcaption{Research articles per year.}
    \label{fig:years}
\end{subfigure}
\\[\baselineskip]
\begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{figures/images/pNumPages2.png}
    \subcaption{Number of pages of articles reporting crowd pilot studies.}%
    \label{fig:pages}%
\end{subfigure}
\end{minipage}%
\end{figure*}




==> figures/FIG-PRISMA.tex <==
{%
\begin{figure*}[!th]%
\centering%
\sffamily
\begin{tikzpicture}[%
    % thick,
    scale=0.44,
    every node/.style={scale=0.44},
    node distance = 6mm and 8mm,
      start chain = A going right,
      base/.style = {draw, minimum width=15mm, minimum height=8mm, align=center, on chain=A},
       txt/.style = {},
  source/.style = {base, minimum width=3cm, rectangle, 
      rounded corners, fill=yellow!30},
  initialsource/.style = {base, rectangle,
      rounded corners, font=\bfseries, fill=yellow!30},
  exclusion/.style = {base, rectangle, rounded corners,
      fill=white!30},
  decision/.style = {base, diamond, fill=green!30},
     final/.style = {base, rectangle, rounded corners, font=\bfseries, fill=red!30},
  every edge quotes/.style = {auto=right}]

\node[initialsource]
    (initialcorpus) {Initial \\ corpus \\ ($n=513$)};            ]
\node[source] [above left=of initialcorpus]
    (acmdl)  {Records identified \\ through database \\ searching (ACM-DL) \\ ($n=300$)};
\node[source] [below left=of initialcorpus]
    (hcomp) {Records identified \\ in HCOMP \\ proceedings \\ ($n=215$)};
\node[exclusion] [right=of hcomp]
    (ex0) {Records \\ unretrievable \\ ($n=2$)};

\node[decision] [right=of initialcorpus]
    (step1) {Keyword \\ ``pilot''?};
\node[exclusion] [above=of step1]
    (ex1) {Records \\ excluded \\ ($n=191$)};

\node[decision] [right=of step1]
    (step2) {Pilot \\ study?};
\node[exclusion] [above=of step2]
    (ex2) {Records \\ excluded \\ ($n=27$)};

\node[decision] [right=of step2]
    (step3) {Pilot \\ conducted?};
\node[exclusion] [above=of step3]
    (ex3) {Records \\ excluded \\ ($n=46$)};

\node[decision] [right=of step3]
    (step4) {Pilot \\ cited?};
\node[exclusion] [above=of step4]
    (ex4) {Records \\ excluded \\ ($n=5$)};

\node[decision] [right=of step4]
    (step5) {Crowd \\ pilot?};
\node[exclusion] [above=of step5]
    (ex5) {Records \\ excluded \\ ($n=56$)};

\node[final] [right=of step5]
    (finalcorpus) {Final \\ corpus \\ ($n=\NUMTOTALARTICLES$)};
%
\node[txt] [below=of step1]
    (text1) {Step 1};
\node[txt] [below=of step2]
    (text2) {Step 2};
\node[txt] [below=of step3]
    (text3) {Step 3};
\node[txt] [below=of step4]
    (text4) {Step 4};
\node[txt] [below=of step5]
    (text5) {Step 5};
%
\draw[arrows=-Stealth] 
    (acmdl) edge[""]         (initialcorpus)
    (hcomp) edge[""]         (initialcorpus)
    (hcomp) edge[""]         (ex0)
    (initialcorpus) edge[""] (step1)
    (step1) edge["present"]  (step2)
    (step2) edge["yes"]      (step3)
    (step3) edge["yes"]      (step4)
    (step4) edge["no"]       (step5)
    (step5) edge["yes"]    (finalcorpus)
    (step1) edge["not present"] (ex1)
    (step2) edge["no"]          (ex2)
    (step3) edge["no"]          (ex3)
    (step4) edge["yes"]         (ex4)
    (step5) edge["no"]          (ex5)
    ;
\end{tikzpicture}%
\caption{Corpus screening procedure.}%
\label{fig:PRISMA}%
\end{figure*}%
}%

==> tables/TAB-CCS.tex <==
% -----
\begin{table}[ht]%
\centering%
\small
\caption{Top-level CCS concepts (with more than 1 occurrence) of articles reporting crowd pilot studies.}%
\label{tab:ccs-concepts}%
\begin{tabularx}{\linewidth}{Xc}
  \hline
\normalsize
 CCS Top-level Concept & \makecell{\normalsize No. of \\ Articles} \\ 
  \hline
  Human-centered computing &  47 \\ 
  Information interfaces and presentation (e.g., HCI) [H.5] &  46 \\ 
  % n/a &  41 \\ 
  Information systems &  26 \\ 
  Computing methodologies &  14 \\ 
  Applied computing &   7 \\ 
  Models and principles [H.1] &   6 \\ 
  Computers and society [K.4] &   6 \\ 
  Information storage and retrieval [H.3] &   5 \\ 
  Software engineering [D.2] &   3 \\ 
  Information systems and applications [H.4] &   3 \\ 
  Social and professional topics &   3 \\ 
  Software and its engineering &   3 \\ 
  Artificial intelligence [I.2] &   2 \\ 
  Image processing and computer vision [I.4] &   2 \\ 
  Pattern recognition [I.5] &   2 \\ 
  Social and behavioral sciences [J.4] &   2 \\ 
  Security and privacy &   2 \\ 
  Theory of computation &   2 \\ 
   \hline
\end{tabularx}
\end{table}
% -----
% \begin{figure}[!h]%
% \customfig{figures/images/pCCSTopLevel.png}{\todo{Top CCS concepts.}}{fig:ccs}%
% \end{figure}%
% -----


==> tables/TAB-Pilotstudies.tex <==
%
% \onecolumn
\begin{table*}[h]%
\centering%
\caption{Research articles reporting crowd pilot studies per year.}%
\label{tab:publications}%
\small%
\begin{tabularx}{.95\textwidth}{lX}%
\toprule%
    Year & Articles \\
\midrule%
    2012 & \input{years/2012} \\
    2013 & \input{years/2013} \\
    2014 & \input{years/2014} \\
    2015 & \input{years/2015} \\
    2016 & \input{years/2016} \\
    2017 & \input{years/2017} \\
    2018 & \input{years/2018} \\
    2019 & \input{years/2019} \\
    2020 & \input{years/2020} \\
    2021 & \input{years/2021} \\
\bottomrule%
\end{tabularx}%
\end{table*}%
% \twocolumn
%

==> tables/TAB-PubDetails.tex <==
\clearpage
\onecolumn

\begin{longtable}[ht]{rlllllllll}
\centering
% \begin{tabularx}{\textwidth}{rlXXXXXXXX}
  \hline
 & Community & Type.of.Section.Consolidated & Type.of.pilot & Crowd & Wording & No..of.pilot.studies.Consolidated & n.workers & n.HITs & remuneration \\ 
  \hline
1 & WebSci & Study/Experiment Design & formative & CrowdFlower/Figure Eight, MTurk & pilot experiment, pilot & $>$1 & n/a & n/a & n/a \\ 
  2 & GamifIR & Study/Experiment Design & formative & MTurk & pilot test & 1 & n/a & n/a & n/a \\ 
  3 & ICTD & (Full paper) & summative & Citizens & pilot community & 1 & n/a & n/a & n/a \\ 
  4 & MM & Pilot Study & summative & Volunteers & pilot project, pilot & 2 & $>$2000 & pilot 1: $>$420,000 tags
pilot 2: $>$750,000 tags & unpaid \\ 
  5 & SIGUCCS & (Full paper) & summative & Volunteers & pilot, pilot phase, pilot implementation & 1 & 200 & $>$50 ideas & raffle (iPad Mini) \\ 
  6 & W4A & Pilot Study & summative & Volunteers & pilot experiment & 1 & 100 / 42 & 578 English video segments & volunteer \\ 
  7 & WWW & System/Workflow/Algorithm & formative & CrowdFlower/Figure Eight & pilot task & 1 & n/a & n/a & n/a \\ 
  8 & ADCS & Study/Experiment Design & formative & MTurk & pilot experiment & 1 & n/a & n/a & n/a \\ 
  9 & CSI-SE & Study/Experiment Design, Limitations & formative, summative & n/a & pilot study, pilot run & $>$1 & n/a & n/a & n/a \\ 
  10 & HCOMP & Study/Experiment Design & formative & MTurk & pilot participant & 2 & 43 + 7 & n/a & n/a \\ 
  11 & ASE & Conclusion & summative & In-house crowdsourcing platform & pilot & 1 & 15 & 15 & n/a \\ 
  12 & CrowdMM & Study/Experiment Design & formative & MTurk & piloting, pilot task & 1 & n/a & 100 & n/a \\ 
  13 & CrowdMM & Pilot Study & formative & Microworkers & pilot & 3 & n/a & n/a & n/a \\ 
  14 & HotMobile & (Full paper) & summative & Elance & pilot study & 1 & 10 & 10 & max. US\$30 \\ 
  15 & Internet-QoE & Study/Experiment Design & formative & Volunteers & pilot study & 1 & 206 & 656 game sessions & unpaid \\ 
  16 & AIES & Results/Evaluation & formative & MTurk & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  17 & BELIV & Study/Experiment Design & formative & MTurk & pilot trial, pilot study & 1 & n/a & n/a & \$0.00...\$8.00 \\ 
  18 & CHI & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  19 & CrowdMM & Pilot Study & formative & Microworkers & pilot, pilot trial & 3 & 120 & 120 & \$0.5, \$0.4, \$0.2 \\ 
  20 & HCOMP & Study/Experiment Design & formative & n/a & pilot study & 1 & n/a & n/a & n/a \\ 
  21 & ISEC & Introduction & summative & Students & pilot implementation & 1 & n/a & n/a & n/a \\ 
  22 & WWW & System/Workflow/Algorithm & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  23 & ASSETS & System/Workflow/Algorithm, Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & approx. \$0.10 per minute \\ 
  24 & ASSETS & (Full paper) & summative & Volunteers & pilot study, pilot & 1 & 3 & $>$93 & n/a \\ 
  25 & CACM & Dataset/Corpus & formative & MTurk & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  26 & CHI & Study/Experiment Design & formative & MTurk & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  27 & CIKM & System/Workflow/Algorithm & formative & MTurk & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  28 & COMPUTE & System/Workflow/Algorithm & formative & n/a & pilot run & 1 & n/a & 36000 tweets & n/a \\ 
  29 & DG-O & (Full paper) & summative & Citizens & pilot & 1 & "almost 40 people" & n/a & unpaid \\ 
  30 & HCOMP & Introduction & formative & MTurk & pilot study & 1 & 106 & 55 workers completed 75 topic tasks (15
HITs with 5 assignments) and 51 workers completed 445
relevance tasks (89 HITs with 5 assignments) & \$0.05 \\ 
  31 & HT & Pilot Study & formative & CrowdFlower/Figure Eight & pilot study & 1 & 100 & 100 & 3.68min x hourly rate of 7USD \\ 
  32 & ICMI & System/Workflow/Algorithm & formative & MTurk & pilot study, pilot test & $>$1 & n/a & n/a & n/a \\ 
  33 & ICMI & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot experiment & 1 & 28 & n/a & n/a \\ 
  34 & AAMAS & System/Workflow/Algorithm & formative, summative & MTurk & pilot study, pilot test & $>$1 & n/a & n/a & n/a \\ 
  35 & AVI & Study/Experiment Design & formative & MTurk & pilot study, pilot & $>$1 & n/a & n/a & n/a \\ 
  36 & HAI & Study/Experiment Design, Discussion & formative & n/a & pilot run, pilot study & 2 & 240 or less & 240 & n/a \\ 
  37 & HCOMP & Pilot Study & formative & MTurk & pilot, pilot study, pilot experiment & 3 & 216 & annotated about 14,000 light curves & average hourly wage:
\$10.993 / \$8.056 / \$4.800 \\ 
  38 & HCOMP & Study/Experiment Design & summative & MTurk, CrowdFlower/Figure Eight & pilot experiment & 2 & 60 & n/a & n/a \\ 
  39 & HCOMP & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot, pilot study & $>$1 & n/a & n/a & n/a \\ 
  40 & HCOMP & Study/Experiment Design & formative & MTurk & pilot test & $>$3 & n/a & n/a & n/a \\ 
  41 & HCOMP & Study/Experiment Design & formative & Students & pilot run, pilot trial & $>$1 & n/a & n/a & n/a \\ 
  42 & HCOMP & Pilot Study & summative & Citizens & pilot & 1 & 29 & $>$7000 reports during the pilot & n/a \\ 
  43 & HCOMP & (Full paper) & summative & Volunteers & pilot study & 1 & 18 & 54 & unpaid \\ 
  44 & NordiCHI & (Full paper) & summative & Volunteers & pilot neighborhood & 4 & 38 & four soundwalks & unpaid \\ 
  45 & WSDM & Study/Experiment Design & formative & Toloka & pilot study & 1 & n/a & n/a & n/a \\ 
  46 & CHI & (Full paper) & summative & Social Media, MTurk, MindSwarms, Kickstarter/IndieGoGo & pilot study, pilot course & 4 & $>$40 & n/a & n/a \\ 
  47 & CHI & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  48 & CHI & System/Workflow/Algorithm & formative & MTurk & pilot testing, pilot run, pilot observation & $>$1 & n/a & n/a & n/a \\ 
  49 & CHI & Study/Experiment Design & formative & MTurk & pilot study & 2 & n/a & n/a & n/a \\ 
  50 & CHI & Study/Experiment Design & formative & MTurk & pilot, piloting & $>$1 & n/a & n/a & n/a \\ 
  51 & CHI & Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  52 & CHI & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot study & $>$1 & n/a & n/a & n/a \\ 
  53 & CHI & Pilot Study & formative & Software Dev Teams & pilot deployment, pilot site & 1 & 168 & n/a & unpaid \\ 
  54 & CHIIR & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot test & 1 & 100 & 100 & n/a \\ 
  55 & CIKM & Dataset/Corpus, Results/Evaluation & formative, summative & MTurk & pilot evaluation, pilot study, pilot & $>$3 & n/a & n/a & n/a \\ 
  56 & CIKM & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot experiment & $>$1 & 3 workers per HIT
+ additional 3-5 per HIT & n/a
3-5 assignments per HIT & US\$0.40 \\ 
  57 & CIKM & Introduction & formative & MTurk & pilot experiment & 1 & 30 & 30 & n/a \\ 
  58 & CIKM & Pilot Study & formative & CrowdFlower/Figure Eight & pilot, pilot study, pilot experiment & $>$3 & 221 & 14160 & \$0.024 \\ 
  59 & CIKM & Pilot Study & summative & Custom platform & pilot study & 1 & 100 & 300 & n/a \\ 
  60 & CSCW & Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  61 & CSCW & System/Workflow/Algorithm & formative & Citizens & pilot test & 1 & 14 & n/a & n/a \\ 
  62 & CSCW & System/Workflow/Algorithm & formative & n/a & pilot testing & n/a & n/a & n/a & n/a \\ 
  63 & DIS & System/Workflow/Algorithm & formative & Citizens & pilot testing & 1 & n/a & n/a & n/a \\ 
  64 & DIS & Study/Experiment Design & formative & MTurk & piloting & n/a & n/a & n/a & n/a \\ 
  65 & HCIR & Study/Experiment Design & formative & Relevance Judgment Platform, MTurk & piloted & 1 & 3 & n/a & n/a \\ 
  66 & HCOMP & Study/Experiment Design & formative & MTurk & pilot & $>$1 & n/a & n/a & n/a \\ 
  67 & HCOMP & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  68 & HCOMP & Pilot Study & formative & MTurk & pilot study, pilot experiment & 1 & n/a & 560 & \$0.05, \$0.10 \\ 
  69 & HCOMP & System/Workflow/Algorithm & formative & MTurk & pilot study, pilot & $>$1 & n/a & n/a & n/a \\ 
  70 & HCOMP & Limitations & formative & CrowdFlower/Figure Eight & pilot run, pilot study & $>$1 & n/a & n/a & n/a \\ 
  71 & HCOMP & Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  72 & HCOMP & Pilot Study & formative & MTurk & pilot survey & 2 & 112 & 112 & \$0.90 per response \\ 
  73 & HCOMP & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  74 & HCOMP & Study/Experiment Design & formative & MTurk & pilot & 1 & n/a & n/a & n/a \\ 
  75 & ICER & Study/Experiment Design & formative & MTurk & pilot test, pilot study & 2 & n/a & 240 & n/a \\ 
  76 & ITS & Dataset/Corpus & formative & CrowdFlower/Figure Eight & piloting, piloted & n/a & n/a & n/a & n/a \\ 
  77 & JCDL & Results/Evaluation & formative & MTurk, UHRS & pilot & 1 & n/a & n/a & n/a \\ 
  78 & SIGIR & Study/Experiment Design & formative & MTurk & pilot study, pilot test, pilot & 1 & 86 & 86 & \$0.05 \\ 
  79 & SIGIR & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot test & 1 & 100 & n/a & n/a \\ 
  80 & SIGIR & Study/Experiment Design & formative & MTurk & pilot, pilot run & $>$1 & n/a & n/a & n/a \\ 
  81 & SIGIR & Pilot Study & summative & MTurk, CrowdFlower/Figure Eight & pilot & 1 & 795 & \~{}4500 & \$0.02 \\ 
  82 & UbiComp & Study/Experiment Design & formative & n/a & pilot study & 1 & n/a & n/a & n/a \\ 
  83 & WebSci & Discussion & summative & MTurk & pilot study & 1 & n/a & n/a & \$0.01 per task \\ 
  84 & WWW & Results/Evaluation & summative & MTurk & pilot study & 1 & 7 & n/a & n/a \\ 
  85 & CHI & Results/Evaluation & formative & MTurk & piloting & n/a & n/a & n/a & n/a \\ 
  86 & CHI & Study/Experiment Design & formative & Citizens & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  87 & CHI & Dataset/Corpus & formative & MTurk & piloting & 1 & n/a & n/a & n/a \\ 
  88 & CHI & Study/Experiment Design, Pilot Study & formative & MTurk & pilot study, pilot & 2 & n/a & n/a & n/a \\ 
  89 & HCOMP & Study/Experiment Design & formative & MTurk & pilot test & $>$1 & n/a & n/a & n/a \\ 
  90 & HCOMP & Study/Experiment Design & formative & Yahoo! crowdsourcing platform & pilot study & 1 & n/a & n/a & n/a \\ 
  91 & WWW & Results/Evaluation & formative & MTurk & pilot experiment, pilot study & 1 & n/a & n/a & n/a \\ 
  92 & WWW & System/Workflow/Algorithm & formative & MTurk & pilot study, pilot test & $>$1 & n/a & n/a & n/a \\ 
  93 & WWW & Study/Experiment Design & formative & MTurk & pilot survey & 1 & n/a & n/a & n/a \\ 
  94 & WWW & System/Workflow/Algorithm & formative & Volunteers & pilot study & $>$1 & n/a & n/a & n/a \\ 
  95 & WWW & Study/Experiment Design & formative & MTurk & pilot study & 1 & 20 & n/a & n/a \\ 
  96 & CHI & Acknowledgements & n/a & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  97 & CHI & System/Workflow/Algorithm & formative & Custom platform & pilot test & $>$1 & n/a & n/a & n/a \\ 
  98 & CHI & Study/Experiment Design & formative & MTurk & pilot testing & $>$1 & n/a & n/a & n/a \\ 
  99 & CHI & Study/Experiment Design & formative & Cint (participant pool) & pilot testing & 1 & n/a & n/a & n/a \\ 
  100 & CHI & Study/Experiment Design & formative & MTurk & pilot & 1 & n/a & n/a & n/a \\ 
  101 & CHI & Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  102 & CHI & Study/Experiment Design & formative & n/a & pilot testing & 1 & n/a & n/a & n/a \\ 
  103 & CHI & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  104 & CHI & (Full paper) & summative & MTurk & pilot & 1 & 98 & n/a & \$0.50 \\ 
  105 & CSCW & System/Workflow/Algorithm & formative & MTurk & pilot analysis & 1 & n/a & n/a & n/a \\ 
  106 & CSCW & System/Workflow/Algorithm & formative & MTurk & pilot study & 1 & n/a & 120 (by n workers)
+ 480 (by one worker) & n/a \\ 
  107 & HCOMP & Results/Evaluation & formative & In-house crowdsourcing platform & pilot, pilot experiment, pilot task & $>$1 & n/a & 55000 & n/a \\ 
  108 & HCOMP & Case Study & summative & MTurk & pilot study & 1 & 109 & 1994 & \$2 / task + \$0.50 bonus \\ 
  109 & HT & Dataset/Corpus & formative & MTurk & pilot study, pilot step, pilot annotation & 1 & 72 & 24 & US \$1.32 \\ 
  110 & TOG & Pilot Study & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  111 & UIST & System/Workflow/Algorithm, Study/Experiment Design & formative & n/a & pilot study, pilot experiment, pilot deployment & $>$1 & n/a & n/a & n/a \\ 
  112 & CHI & Study/Experiment Design & formative & MTurk & pilot study & 1 & 98 & 980 & n/a \\ 
  113 & CHI & Study/Experiment Design, Discussion & formative & MTurk & pilot, piloting & $>$1 & n/a & n/a & n/a \\ 
  114 & CHI & System/Workflow/Algorithm & formative & MTurk & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  115 & CHI & Study/Experiment Design & formative & MTurk & piloted & 1 & n/a & n/a & n/a \\ 
  116 & CHI & System/Workflow/Algorithm & formative & MTurk & pilot, pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  117 & CHI & Study/Experiment Design & formative & Prolific & pilot study & 1 & 10 & n/a & n/a \\ 
  118 & CHI & (Full paper) & summative & MTurk & pilot study & 1 & 33 & 3 assignments per sample & "UK minimum wage" \\ 
  119 & MUM & Study/Experiment Design & formative & Prolific & piloted & 1 & 3 & n/a & n/a \\ 
  120 & CHI & System/Workflow/Algorithm & formative & MTurk & pilot study, pilot & $>$1 & n/a & n/a & n/a \\ 
  121 & CHI & System/Workflow/Algorithm & summative & MTurk & pilot testing & n/a & n/a & n/a & n/a \\ 
  122 & CHI & Study/Experiment Design & formative & MTurk & piloting & 1 & n/a & n/a & n/a \\ 
  123 & CSCW & System/Workflow/Algorithm & formative & Students & pilot study & 1 & 900 & n/a & n/a \\ 
  124 & CSCW & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot & $>$1 & n/a & n/a & n/a \\ 
  125 & TOG & Study/Experiment Design, Appendix & summative & MTurk & pilot study & 1 & 55 & 250 & n/a \\ 
  126 & UIST & Case Study & summative & Students, Researchers, Industry professionals & pilot experiment & 1 & n/a & n/a & n/a \\ 
  127 & CSCW & Results/Evaluation & summative & CrowdFlower/Figure Eight & pilot study & 1 & 86 & 86 & n/a \\ 
  128 & UIST & System/Workflow/Algorithm, Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  129 & UIST & Study/Experiment Design & formative & LabInTheWild & pilot study & $>$1 & n/a & n/a & n/a \\ 
  130 & CHI & Study/Experiment Design & formative & MTurk & pilot experiment, piloting & 2 & n/a & n/a & n/a \\ 
  131 & OOPSLA & System/Workflow/Algorithm, Pilot Study, Study/Experiment Design, Results/Evaluation & formative & MTurk & pilot study, pilot test & $>$1 & n/a & n/a & n/a \\ 
  132 & CHI & Limitations & summative & Clickworker & pilot study & 1 & n/a & n/a & n/a \\ 
  133 & CHI & Study/Experiment Design & formative & Prolific & pilot & $>$1 & n/a & n/a & n/a \\ 
  134 & CSCW & Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  135 & CSCW & System/Workflow/Algorithm,
Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  136 & IMWUT & Study/Experiment Design & n/a & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  137 & TAP & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot study, pilot & 1 & n/a & n/a & n/a \\ 
  138 & TIST & System/Workflow/Algorithm, Study/Experiment Design & formative & MTurk & pilot study, pilot test & 1 & n/a & n/a & \$0.15...\$0.50 \\ 
  139 & CSCW & Study/Experiment Design & formative & MTurk & pilot experiment, pilot study & 1 & n/a & n/a & n/a \\ 
  140 & TIST & Study/Experiment Design & formative & MTurk & pilot experiment & $>$1 & n/a & n/a & n/a \\ 
  141 & TOIS & System/Workflow/Algorithm & formative & MTurk & pilot study, pilot test & $>$1 & n/a & 3743 minus 2498 & n/a \\ 
  142 & CSCW & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  143 & CSCW & Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot study & 1 & n/a & n/a & n/a \\ 
  144 & CSCW & Pilot Study & formative & MTurk & pilot study, pilot test, pilot & 3 & 33 & n/a & n/a \\ 
  145 & CSCW & (Full paper) & summative & Older adults & pilot study, pilot, pilot evaluation & 1 & 7 & n/a & n/a \\ 
  146 & TACCESS & System/Workflow/Algorithm, Study/Experiment Design & formative & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  147 & CSCW & Appendix & formative & MTurk & pilot study, pilot & 1 & 50 & 50 & \$10 \\ 
  148 & CSCW & Study/Experiment Design & formative & MTurk & pilot study & 1 & n/a & n/a & n/a \\ 
  149 & IMWUT & Case Study & summative & Students & pilot & 1 & 325 & $>$242 & n/a \\ 
  150 & CSCW & Pilot Study, Appendix & formative & MTurk & pilot study, pilot test, pilot experiment & 1 & n/a & n/a & n/a \\ 
  151 & JOCCH & Results/Evaluation & summative & n/a & pilot crowdsourcing study, pilot set & 1 & 10 annotators per task & 1000 annotations & USD \$ 0.10 per page (4 tasks) \\ 
  152 & TIST & System/Workflow/Algorithm & formative & Custom platform & pilot study & 1 & 5 & n/a & n/a \\ 
  153 & CSCW & Study/Experiment Design & formative, summative & MTurk & pilot study, pilot & $>$1 & n/a & n/a & n/a \\ 
  154 & CSCW & Dataset/Corpus, Discussion & formative & MTurk & pilot study & $>$3 & n/a & n/a & n/a \\ 
  155 & TOIT & Discussion & formative & CrowdFlower/Figure Eight & pilot experiment & 1 & n/a & n/a & USD \$0.10 down to USD \$0.05 \\ 
  156 & CSCW & Study/Experiment Design, Limitations & formative & CrowdFlower/Figure Eight & pilot study & 1 & n/a & n/a & n/a \\ 
  157 & EICS & System/Workflow/Algorithm & summative & n/a & pilot-tested & 1 & n/a & n/a & n/a \\ 
  158 & TIST & System/Workflow/Algorithm, Study/Experiment Design & formative & CrowdFlower/Figure Eight & pilot & 1 & n/a & n/a & n/a \\ 
  159 & IMWUT & Abstract & formative & CrowdFlower/Figure Eight & pilot study & 1 & 100 & 100 & \$7.5 \\ 
  160 & TOIS & Study/Experiment Design & n/a & MTurk & pilot study & $>$1 & n/a & n/a & n/a \\ 
  161 & TWEB & System/Workflow/Algorithm & formative & MTurk & pilot study, pilot testing, pilot annotations, pilot test & $>$1 & 218 & 10 assignments per task & USD\$6 per task \\ 
  162 & CSCW & System/Workflow/Algorithm & formative & MTurk & pilot task & 1 & n/a & n/a & n/a \\ 
  163 & TOCHI & Study/Experiment Design & summative & MTurk & pilot study, pilot & 2 & 24, n/a & n/a & n/a \\ 
  164 & TSC & Background/Related Work, Study/Experiment Design, System/Workflow/Algorithm & formative & CrowdFlower/Figure Eight & pilot & $>$1 & n/a & n/a & n/a \\ 
  165 & IMWUT & Results/Evaluation & summative & postal workers & pilot, pilot study & 1 & 10 & 682 responses & unpaid \\ 
  166 & TOCHI & Study/Experiment Design & formative & MTurk & pilot experiment & $>$1 & n/a & $>$ 19, $>$ 11 & n/a \\ 
  167 & CHI & System/Workflow/Algorithm, Study/Experiment Design, Appendix & formative & MTurk & pilot study, pilot & $>$1 & n/a & n/a & n/a \\ 
  168 & JDIQ & Appendix & formative & MTurk & pilot & 1 & n/a & n/a & n/a \\ 
  169 & TOIS & Study/Experiment Design, Limitations & formative & MTurk & pilot test, pilot testing & n/a & n/a & n/a & n/a \\ 
  170 & GROUP & Study/Experiment Design & formative & ZBJ & pilot test, pilot study & 1 & 14 & n/a & n/a \\ 
  171 & TOCHI & Study/Experiment Design & formative & MTurk & pilot experiment, pilot & $>$1 & n/a & n/a & n/a \\ 
   \hline
% \end{tabularx}
\end{longtable}
